Inferential Tasks as an Evaluation Technique for Visualization

Designing suitable tasks for visualization evaluation remains challenging. Traditional evaluation techniques commonly rely on 'low-level' or 'open-ended' tasks to assess the efficacy of a proposed visualization, however, nontrivial trade-offs exist between the two. Low-level tasks allow for robust quantitative evaluations, but are not indicative of the complex usage of a visualization. Open-ended tasks, while excellent for insight-based evaluations, are typically unstructured and require time-consuming interviews. Bridging this gap, we propose inferential tasks: a complementary task category based on inferential learning in psychology. Inferential tasks produce quantitative evaluation data in which users are prompted to form and validate their own findings with a visualization. We demonstrate the use of inferential tasks through a validation experiment on two well-known visualization tools.

==> contents/sec-background.tex <==
\section{Motivation}

The principle behind the use of inferential tasks is rooted in inferential learning from psychology research. Inferential learning is learning that occurs through \textit{thinking}, particularly through inductive, deductive, and abductive reasoning\cite{seel2012inferential}. In inferential learning, a learner can \textit{infer} new knowledge and information through logical reasoning, even if the learner has no first-hand experience of observing that information. 

The process of inferential learning can be strongly related to visual data exploration. Data analysts often need to infer knowledge from observing and reasoning about data to satisfy a set of analyses goals. For example, an analyst might observe a data point that appears different from others in a visualization and hypothesize that this data point is an outlier. However, upon further exploration of the data, the analyst might refute the hypothesis because they discover additional data points that share the same characteristic. 

Our motivation for proposing the use of inferential tasks in evaluation is based on the above observation -- that visual analysis tasks are similar in nature to inferential learning. Given that the goal of visual data analysis is to infer new knowledge and insights through data exploration\cite{north2006toward}, we find it logical to design an evaluation task based on inferential learning. By definition, inferential tasks can assess participants' ability to use a visualization to perform the same reasoning steps as those used in visual data analysis.

\begin{figure}[h!]
\centering %left bot right top
%  \fbox{
 \includegraphics[clip, trim=0 5.5cm 9.6cm 0, width=.85\linewidth]{figures/itask_example.pdf} %}
\caption{\textit{Illustrative visualization tool that supports users in the exploration of monthly item sales for a specified year.}
 }
     \label{fig:inferentialTaskExample}
\end{figure}

==> contents/sec-old-introduction.tex <==
\section{Introduction}
% \label{sec:intro}

When evaluating visualization systems, numerous approaches have been suggested over the years to ascertain both the benefits and limitations of a proposed tool\cite{brehmer2013multi, burns2020evaluate}.
Central to these approaches is the design of the \textit{tasks} that users are asked to perform while using a visualization. Measuring and observing a user's performance on these tasks provides the basis for evaluating the effectiveness of a visualization's intended use\cite{sedlmair2012dsm, lam2012empirical}.

However, despite the numerous task taxonomies proposed by the visualization community, most user studies rely on two task \textit{types} when evaluating visualizations: low-level, `fact-acquisition' tasks (e.g., for controlled benchmark experiments), and high-level, `open-ended' tasks (e.g., for think-aloud protocols)\cite{saraiya2005insight}.
The benefits and popularity of these evaluation task types are well documented\cite{chen2000empirical}, yet, there exists a non-trivial trade-off between the two. 
Fact-acquisition tasks, although straightforward to implement and analyze, produce evaluation data that is not representative of a visualization's insight and knowledge capabilities\cite{kosara2016empire}.

When these factors are crucial to the assessment of a visualization, evaluation designers may rely on open-ended tasks in an interview-style ``qualitative insight analysis'' evaluation\cite{north2006toward, carpendale2008evaluating}. The benefits of an evaluation with qualitative tasks are indisputable\cite{ali2012qualitative, peck2019personal, meyer2019criteria}. However, conducting and analyzing feedback from these think-aloud tasks through interviewing and open-coding is a time-consuming endeavor that is not always feasible or scalable for the designer\cite{anderson2010presenting}. 

In this paper, we formalize a new class of evaluation tasks that serve as a complement to both fact-acquisition and open-ended tasks: \textit{Inferential tasks}.
% Inspired by the concept of inferential learning from psychology and education literature\cite{seel2012inferential}, 
Inferential tasks require evaluation participants to construct knowledge by inferring relations between learned concepts and new observations, engaging users in a pattern of analysis similar to open-ended visualization tasks. 
% As a result, users engage in a similar pattern of analysis as when performing open-ended visual analysis tasks -- forming new insights based on observed relations in the data. 
Moreover, inferential tasks can be set up with clear `correct' or `incorrect' answers, resulting in quantitative evaluation data that can be analyzed with the same statistical methods as low-level task evaluations. 
% As a result, the evaluation data produced by inferential tasks allows designers to benchmark a more complex pattern of analysis that is closer to open-ended visual analysis tasks. 

Inferential tasks have been used with success in visualization evaluation previously. Green et al\. and Ziemkiewicz et al\. showed that tasks that involve inferential learning produce more nuanced and informative evaluation data than tasks that only involve \textit{procedural learning} (i.e., low-level tasks)\cite{green2010using, ziemkiewicz2011locus}. Though the authors share these finding in their work, they do not offer a formalization or design methodology for inferential task evaluations.   In this paper, we present the first formalization of inferential tasks in visualization literature. 

We demonstrate how inferential tasks can be deployed in practice in a validation experiment comparing two well-known exploratory visualization tools, Voyager 2\cite{2017-voyager2} and Polestar\cite{2016-voyager}. Our results indicate that the use of inferential tasks produce evaluation data that illuminates differences between the tools, while remaining straightforward to analyze quantitatively. Finally, we discuss considerations and limitations for deploying inferential tasks in visualization evaluations, and outline future work for their design.
